Compositional Exemplars for In-context Learning

Large pretrained language models (LMs) have shown impressive In-Context Learning (ICL) ability, where the model learns to do an unseen task via a prompt consisting of input-output examples as the demonstration, without any parameter updates. The performance of ICL is highly dominated by the quality of the selected in-context examples. However, previous selection methods are mostly based on simple heuristics, leading to sub-optimal performance. In this work, we formulate in-context example selection as a subset selection problem. We propose CEIL (Compositional Exemplars for In-context Learning), which is instantiated by Determinantal Point Processes (DPPs) to model the interaction between the given input and in-context examples, and optimized through a carefully-designed contrastive learning objective to obtain preference from LMs. We validate CEIL on 12 classification and generation datasets from 7 distinct NLP tasks, including sentiment analysis, paraphrase detection, natural language inference, commonsense reasoning, open-domain question answering, code generation, and semantic parsing. Extensive experiments demonstrate not only the state-of-the-art performance but also the transferability and compositionality of CEIL, shedding new light on effective and efficient in-context learning. Our code is released at https://github.com/HKUNLP/icl-ceil.

==> tabs/scale.tex <==
\begin{table}[t]
\centering
\caption{Comparisons of different trade-off factors for balancing relevance and diversity of in-context examples.}
\label{tab:scale}
\vskip 0.15in
\scalebox{0.7}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Method} & \multicolumn{1}{c}{\textbf{SST5}} & \multicolumn{1}{c}{\textbf{MRPC}} & \multicolumn{1}{c}{\textbf{MNLI}} & \multicolumn{1}{c}{\textbf{WebQs}} & \textbf{NL2Bash} & \multicolumn{1}{c}{\textbf{MTOP}} \\
\midrule
\multicolumn{7}{l}{\textit{Baselines}} \\
\textsc{TopK-BERT} & 37.24 & 69.36 & 42.15 & 17.08 & 51.30 & 52.13 \\
\textsc{EPR} & 42.82 & 75.98 & 66.06 & 19.59 & 56.82 & 64.20 \\
\multicolumn{7}{l}{\textit{Trade-off factor $\lambda$}} \\
0.01 & \textbf{47.05} & 78.68 & 70.25 & \textbf{20.92} & 57.84 & 66.71 \\
0.05 & 46.14 & 79.90 & 71.36 & 20.18 & \textbf{59.91} & \textbf{67.43} \\
0.1 & 43.32 & \textbf{80.15} & \textbf{71.74} & 19.44 & 57.30 & 66.58 \\
\bottomrule
\end{tabular}}
\end{table}
